Graph-Induced Syntactic-Semantic Spaces in Transformer-Based Variational AutoEncoders

The injection of syntactic information in Variational AutoEncoders (VAEs) has been shown to result in an overall improvement of performances and generalisation. An effective strategy to achieve such a goal is to separate the encoding of distributional semantic features and syntactic structures into heterogeneous latent spaces via multi-task learning or dual encoder architectures. However, existing works employing such techniques are limited to LSTM-based VAEs. In this paper, we investigate latent space separation methods for structural syntactic injection in Transformer-based VAE architectures (i.e., Optimus). Specifically, we explore how syntactic structures can be leveraged in the encoding stage through the integration of graph-based and sequential models, and how multiple, specialised latent representations can be injected into the decoder's attention mechanism via low-rank operators. Our empirical evaluation, carried out on natural language sentences and mathematical expressions, reveals that the proposed end-to-end VAE architecture can result in a better overall organisation of the latent space, alleviating the information loss occurring in standard VAE setups, resulting in enhanced performances on language modelling and downstream generation tasks.

==> sections/limitations.tex <==
\section*{Limitations}
Despite the increased degree of separability and generation control achieved for the explanatory sentences by flow-based INN, it is only the first step into connecting disentangled semantic roles. How to achieve natural language inference through this latent space with geometric properties still needs to be explored.

==> tables_new/decoding_recon.tex <==
% \begin{center}
\begin{table}[ht!]
\scriptsize
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
\small
\centering
\renewcommand\arraystretch{1.2}
\begin{tabular}{lcccccccccc}
\toprule
Test sets & \multicolumn{2}{c}{EVAL} & \multicolumn{2}{c}{SWAP} & \multicolumn{2}{c}{EASY} & \multicolumn{2}{c}{EQ} & \multicolumn{2}{c}{LEN} \\ 
Metrics & EM & Bleu & EM & Bleu & EM & Bleu & EM & Bleu & EM & Bleu \\ \hline

\multicolumn{11}{c}{\textit{baselines}} \\
AAE(768) & & 0.75 & 0.00 & 0.25 & & 0.53 & 0.00 & 0.54 & & 0.51 \\
LAAE(768) & & 0.43 & 0.00& 0.25 & & 0.27 & 0.00& 0.29 & & 0.44 \\
DAAE(768) &  & 0.24 & 0.00& 0.21 & & 0.21 & 0.00& 0.22 & & 0.42\\
$\beta$-VAE(768) & & 0.14 & 0.00& 0.15 & & 0.13 & 0.00 & 0.14 & & 0.35 \\
Optimus(768) & & 0.99 & 0.00 & 0.38 & 0.81 & 0.93 & 0.00& 0.81 & & 0.76 \\  \hdashline
Bert-GraphSAGE & & 0.96 & 0.00 & 0.28 & 0.06 & 0.46 & 0.00& 0.69 & & 0.60 \\
+ sep dec & \\
+ sep attn & \\
+ fuse query & \\
Bert-TransConv & & 0.95 & 0.00& 0.28 & 0.14 & 0.53 & 0.00& 0.67 & & 0.60 \\
+ sep dec & \\
+ sep attn & \\ 
+ fuse query & \\ \hline
\end{tabular}
}
\caption{Symbolic language modelling.} \label{tab:decoding_recon}
\end{table}
% \end{center}

==> tables_new/stat_data.tex <==
\begin{table}[ht!]
    \small
    \centering
    \renewcommand\arraystretch{1}
      % \resizebox{7.6cm}{!}{
    \begin{tabular}{|c|cc|}
        \hline
        Corpus & Num data. & Avg. length \\ \hline
        WorldTree & 11430 & 8.65 \\
        EntailmentBank & 5134 & 10.35 \\ 
        Math Symbol & 32000 & 6.84 \\
        Math Symbol Inference & 32000 & 51.84 \\ \hline
        
    \end{tabular}
    % }
    \caption{Statistics from datasets.} \label{tab:stats_data}
\end{table}
